Tin-Tin: Towards Tiny Learning on Tiny Devices with Integer-based Neural Network Training

Recent advancements in machine learning (ML) have enabled its deployment on resource-constrained edge devices, fostering innovative applications such as intelligent environmental sensing. However, these devices, particularly microcontrollers (MCUs), face substantial challenges due to limited memory, computing capabilities, and the absence of dedicated floating-point units (FPUs). These constraints hinder the deployment of complex ML models, especially those requiring lifelong learning capabilities. To address these challenges, we propose Tin-Tin, an integer-based on-device training framework designed specifically for low-power MCUs. Tin-Tin introduces novel integer rescaling techniques to efficiently manage dynamic ranges and facilitate efficient weight updates using integer data types. Unlike existing methods optimized for devices with FPUs, GPUs, or FPGAs, Tin-Tin addresses the unique demands of tiny MCUs, prioritizing energy efficiency and optimized memory utilization. We validate the effectiveness of Tin-Tin through end-to-end application examples on real-world tiny devices, demonstrating its potential to support energy-efficient and sustainable ML applications on edge platforms.

==> 01_intro.tex <==
\section{Introduction}
\jinhang{Working on a revision of the intro... will update it soon.}
The rapid development of the Internet of Things (IoT) and edge computing has significantly expanded the deployment of machine learning (ML) on edge devices, thereby enhancing the efficiency and responsiveness of applications like wearable sensing~\cite{nyamukuru2020tinyeats,liu2023realtime,jeyakumar2019senseHAR} and smart cities~\cite{khan2020edge,chen2021edge,alahi2023integration}. Moreover, many emerging applications, such as wildfire monitoring~\cite{bushnaq2021role,liu2021sensor} and earthquake detection~\cite{abdalzaher2021deep,zainab2023lighteq}, necessitate maintenance-free, long-lived sensor networks~\cite{lorincz2009mercury,hester2017future,sparks2017route} that can deploy ML models to detect anomalies and make predictions about the environment. In these scenarios, low-power sensors and microcontrollers (MCUs) play a critical role, being both cost-effective and disposable, to ensure sustainability and longevity.
% Old version
% Driven by the rapid development of the Internet of Things (IoT) and edge computing, integrating machine learning (ML) with low-power edge sensors in these systems has become essential to enhance efficiency and responsiveness in applications such as wearable devices~\cite{nyamukuru2020tinyeats,liu2023realtime,jeyakumar2019senseHAR} and hazard event detection~\cite{zainab2023lighteq}.
% Low-power sensors and microcontrollers (MCUs) are crucial for sustaining  maintenance-free and long-lived sensor networks~\cite{lorincz2009mercury,hester2017future,sparks2017route}. Additionally, these devices are cost-effective and disposable, making them ideal for large-scale, resilient sensor systems in scenarios like wildfire~\cite{bushnaq2021role,liu2021sensor} and earthquake detection~\cite{abdalzaher2021deep,abdalzaher2023employing}.

However, enabling ML on these resource-constrained devices presents new challenges. Power-efficient MCUs typically have limited memory and computing capabilities, as detailed in Sec. \ref{sec:memory_mot}. For instance, the popular STM32 Cortex M0\footnote{https://www.st.com/en/microcontrollers-microprocessors/stm32f0-series.html} MCUs have up to 144 KB of data RAM, and the MSP430\footnote{https://www.ti.com/microcontrollers-mcus-processors/msp430-microcontrollers/overview.html} mixed-signal MCUs offer up to 66 KB. In addition to memory constraints, both lack dedicated floating point units (FPUs), which are designed to handle  operations on floating point numbers. Consequently, these MCUs can only perform integer arithmetic or rely on slow software implementations for floating-point calculations. These limitations significantly restrict the complexity of ML models that can be deployed on these devices, particularly when their battery life is also limited.
Additionally, most prior work on edge ML only focuses on inference. However, in real-world setups such as ad-hoc or personalized sensing~\cite{pan2010transfer}, on-device training is crucial because devices need to dynamically learn new tasks and continuously adapt to changing input distributions.
For example, continuously learning new location information for indoor WiFi localization can significantly reduce recalibration efforts, but this requires efficient resource management to prevent rapid battery drain. %(\bob{this sentence is vague -- give an example to motivate the importance of on-device learning for low power edge})
\carlee{once the applications are finalized, put them as examples here}


\begin{table*}
    \caption{Related Work and Comparison.  %\carlee{maybe add a column on whether it's deployed on microcontrollers and/or under power constraints, to better contrast with NITI}
    }
    \label{tab:related_compare}
    \begin{center}
    \begin{tabular}{l l l l l l l l }\toprule
         &  \makecell[cl]{Optimization\\Target} & \makecell[cl]{Applied\\Stage} & \makecell[cl]{Pre-runtime\\Data Not\\Required} & \makecell[cl]{Integer\\Backprop} &\makecell[cl]{Dynamic\\Weight\\Range} & \makecell[cl]{Low-Power\\MCU\\Deployment} \\\midrule
         % QAT& model quantization & training & \makecell[cl]{inference\\performance} & yes & yes\\\hline
       \makecell[cl]{Model compression\\\& optimization\\\cite{han2015deep,jacob2018quantization,gysel2018ristretto,fedorov2019sparse,lin2020mcunet}} & \makecell[cl]{network,\\layers,\\connections} & \makecell[cl]{post-training,\\training${^*}$}  & no & no & N/A & M7~\cite{lin2020mcunet} \\\hline
        \makecell[cl]{Sparse update \\~\cite{lin2022ondevice,profentzas2022minilearn,wang2019e2train,kwon2024tinytrain,huang2023elastic}} & \makecell[cl]{backward\\layers, \\connections}  & \makecell[cl]{pre-runtime,\\runtime} & no & \makecell[cl]{\cite{wang2019e2train}} & N/A &\makecell[cl]{M7~\cite{lin2022ondevice}\\M4~\cite{profentzas2022minilearn}} \\\hline
        \makecell[cl]{Reduced-precision\\training~\cite{zhu2016trained,li2022ternary}} & \makecell[cl]{arithmetic,\\data } & runtime  & yes/no & no & no & N/A\\\hline
        NITI~\cite{wang2022niti} & \makecell[cl]{arithmetic,\\data}  & runtime & \textcolor{darkgreen}{{yes}} & \textcolor{darkgreen}{{yes}} & no & N/A \\\hline
        Ours & \makecell[cl]{arithmetic,\\data}  & runtime  & \textcolor{darkgreen}{{yes}} & \textcolor{darkgreen}{{yes}} & \textcolor{darkgreen}{{yes}}  & \textcolor{darkgreen}{M0, M4} \\\hline
    \end{tabular}
    \end{center}
    \footnotesize\emph{$^*$} The term ``training'' is used separate from ``runtime'' to emphasize the clear distinction between model training phase and the inference phase in these works. 
    
    \footnotesize\emph{Note:} ``M'' in the last column refers to the Cortex M series. 
\end{table*}


Our goal is to support and optimize \emph{tiny, lifelong} data learning on these \emph{highly constrained} low-power sensor devices with only hundreds of KB memory while extending battery life. Training, compared to pure inference, involves significantly more memory and computational loads (Sec. \ref{sec:memory_mot},\ref{sec:int-motive}), taking approximately $7\times$ longer time than inference~\cite{xu2022mandheling} in app xxx. \carlee{say something about power usage too, since that is one of our primary metrics}
%Even training shallow neural networks can be compute-heavy and memory-intensive, overwhelming inexpensive edge sensors that lack FPUs or parallel processing.  For example, matrix multiplication of two 10x10 matrices requires  1000 multiply and accumulate operations (MACs), with training requiring at least 3× more MACs than inference~\cite{xu2022mandheling}. \jinhang{The relationship between matrix multiplication and training/inference is unclear.}
In order to improve energy efficiency \carlee{in lifelong learning}, one promising solution is to replace full-precision floating points with reduced-precision low-bitwidth data types, which decrease memory requirements by using smaller data formats (e.g., \texttt{fp32} to \texttt{int8}) and simplify calculations (e.g., floating point to integer arithmetic). \carlee{mention that this solution fits well with the lack of FPUs mentioned above} This reduction  complements \carlee{existing} structure- and network-level optimizations like sparse updates~\cite{lin2022ondevice} and pruning~\cite{liu2019metapruning}, benefiting shallow networks as well. \carlee{what does this have to do with shallow networks? Do you mean that sparse updates don't benefit shallow networks as much since there isn't much to optimize?}
% \carlee{Since sensor networks are mentioned earlier, we should mention communication, to convey inferences at the very least, and make the argument that training operations are a significant source of energy usage. perhaps also mention distributed/federated frameworks here (and say that on-device training benefits them too)}

\carlee{condense this paragraph and say here that ours is the first work to do truly integer-based on-device training for low-power MCUs} Despite efforts like TinyML \cite{unite-ai2023tinyml,banbury2021benchmarking} and model compression techniques \cite{han2015deep,wang2019haq,basu2019qsparse,liberis2021munas} \carlee{to reduce the energy usage and computational overhead of on-device model deployment [is this true?]}, gaps remain in achieving low-power, adaptable \carlee{``lifelong learning'' instead of adaptable?} applications. These methods are effective for inference but cannot handle model updates.  Memory-efficient on-device deep neural network (DNN) training can be achieved through sparse updates \cite{lin2022ondevice,profentzas2022minilearn,qu2022p,huang2023elastic} or by trading off more computation for lower memory usage \cite{pan2021mesa,gim2022memory,wang2022melon,patil2022poet}. However, \carlee{existing methods} require pre-runtime training with extensive search and pruning or incur significant computation overhead~\cite{kwon2024tinytrain}.  Reduced-precision models and weight updates \cite{bernstein2018signsgd,courbariaux2015binaryconnect,zhu2016trained,li2022ternary} still require heavy intermediate floating-point calculations, and some rely on non-standard dedicated hardware. In contrast, using integer arithmetic reduces hardware complexity and improves energy efficiency~\cite{wang2022niti}, as standard integer arithmetic units are widely available. For a detailed summary of related work, see Table \ref{tab:related_compare} and Sec. \ref{sec:related}.

This work aims to use integer operands for the majority of neural network training calculations, addressing two main \textbf{technical challenges}: 

{ \textbf{Dynamic Range Requirements.} } Using integer arithmetic for neural network training requires integer operands, including weights ($w$), activations ($a$), gradients ($g$) and errors ($e$) for all computations, such as multiplying $w$ and $a$. Unlike floating points, which have a wide representable range  (e.g., $1.4$e$^{-45}$ to $3.4$e$^{38}$ for \texttt{float32}), integers have a limited range (e.g., $[-128,127]$ for \texttt{int8}). Fixed ranges based on presumed value limits can lead to overflow (unwanted clipping) or reduced precision (Sec. \ref{sec:dr_motivation}). To maintain accuracy, value ranges should be dynamically adjusted during training, as the distributions of inputs, outputs, and weights change. This dynamic adjustment  improves model performance by ensuring appropriate scaling throughout the training process. We introduce an integer-based rescaling scheme that dynamically adjusts the value ranges without introducing heavy floating point operations. 


%Thus, a dynamic range is required to maintain high numerical accuracy during training,  ensuring that the values remain within representable limits without sacrificing precision.



{\textbf{Integer Weight Update.}} Maintaining accurate model updates with integer weights is challenging due to their limited precision. The desired update values often need to be much smaller (a tenth or a hundredth) than the weights themselves. Traditional gradient descent techniques achieve this by using a small learning rate (e.g., 0.001) to scale down the gradient update, guiding the model towards the optimum. However, in integer-based training, directly applying a small learning rate is problematic because multiplying integer gradients by a small scalar produces floating-point values. Converting these scaled floating-point gradients back to integers introduces additional computational costs and precision issues. Therefore, innovative methods are required to apply integer gradient updates that are much smaller in scale than the weights, while maintaining accuracy within the integer-only framework.

To address these challenges and target resource-constrained sensor devices,  our integer-based training framework incorporates the following \textbf{novel techniques}: \carlee{elaborate on how these solve the challenges above. These could also be combined with the contributions list}
\begin{itemize}
    \item \textbf{Integer-Based Rescaling}
    \item \textbf{Lightweight Range Adjustment Scheme}
    \item \textbf{Efficient Weight Update Schedule}
\end{itemize}
 \carlee{Is a power analysis of integer training also novel? If we can say something about designing and thoroughly evaluating an end-to-end framework, that would also be a nice contribution and way to differentiate ourselves from NITI.}

\paragraph{Contributions}
In summary, we propose an integer-based neural network training framework designed for tiny learning tasks on resource-constrained sensor devices. We extend the NITI framework to support dynamic range. \carlee{Instead of the last sentence, I would say something like ``We introduce novel integer rescaling techniques that support a dynamic range and efficient weight updates, and we demonstrate our framework's effectiveness in end-to-end application examples on tiny devices.''}
%\carlee{``extend'' suggests that our work doesn't add much to NITI. I think it is better to say that, while NITI solves some of the basic challenges of integer-based training, it leaves several crucial questions unanswered, which are particularly important for power-limited devices (as far as I can tell, NITI is designed more for GPUs and FPGAs).} 
The main contributions are:
\begin{itemize}
\item (Section~\ref{sec:system}) We design and implement an integer-based neural network training framework.  
\item (Section~\ref{}) Our solution offers dynamic range support through efficient integer-only rescaling and efficient range adjustment scheme.
\item (Section~\ref{}) We devise an efficient weight update mechanism. 
\item We evaluate the framework on diverse learning applications and perform a case study on a real-world small-scale system. 
\end{itemize}


==> 04_FL.tex <==
\subsection{\texttt{FedDiff}}\label{sec:feddiff}

In this section, we present FedDiff, our federated training algorithm. We first introduce the formal FL optimization problem and then describe FedDiff's design.

Due to the asynchronous nature of our system (introduced in Section \ref{sec:system}), and to lower the volume of data to be communicate, we send the quantized  and sparse model difference from the client to the server, instead of sending the entire model parameters . Based on these techniques and to fit within the system's extreme resource constraints, we propose the \texttt{FedDiff} algorithm, which is shown in Algorithm \ref{alg:FedDiff}.

In FedDiff, every client and server initializes its model with parameter $X_0$. Within each round of communication, each client simultaneously updates its local model by running several steps of gradient descent. We suppose that the number of local gradient descent epochs and batch size is predefined by the central server, as is typical in federated learning~\cite{mcmahan2017fedavg}. Before doing any local updates, each client $n$ stores its current model parameters as $X_{n0}$. In each local epoch, each local client $n$ performs a step of batch gradient decent and updates its local model parameters $X_n$ according to the following equation:

\begin{equation}
    X_n \leftarrow X_n - \eta \nabla l(X_n; b)
\end{equation}
where $\eta$ is a pre-defined learning rate.
Each client is then scheduled to communicate with the server to exchange parameters. The order in which the clients communicate with the server can be scheduled by the network base station by pre-specifying times at which the clients should wake up and begin transmitting a model update.
%is based on the asynchronous scheme we selected (see Section \ref{sec:system}). 
For example, this order can be cyclic, uniformly random, etc.

During the parameter exchange stage, the scheduled client first computes the model difference $\Delta X\equiv X_n - X_{n0}$. It then sparsifies $\Delta X$ by dropping parameter differences that are smaller than a certain (given) threshold. Since these are not transmitted to the server, this thresholding decreases the amount of data to be transmitted.  While this sparse update is being transmitted to the server, the server simultaneously sends the current global model $X_c$ to the client, using the Feather-COMM protocol. After the selected client and the server received the model parameters, they then update their model parameters according to the following equation:
\begin{equation}
\begin{aligned}
    \text{server:  } & X_c \leftarrow X_c + \frac{\Delta X}{N} \\
    \text{client:  } & X_n \leftarrow X_c + \frac{\Delta X}{N} 
\end{aligned}
\end{equation}

This update guarantees that the most recent global model aligns with the current local model, while minimizing the amount of data to be sent and shortening the time required for the parameter exchange. 
%
This process repeats iteratively until the pre-set maximum number of iterations $T$ is reached or the model converges.

\begin{algorithm}
\caption{\texttt{FedDiff}: There are $N$ clients indexed by $n$, $\eta$ represents the learning rate, $B$ is the batch size, $E$ is the number of local epoch.}
\label{alg:FedDiff}
\begin{algorithmic}[1]
\State \textbf{Server stores:}
\State Server model parameter: $X_c$
\Statex
\State \textbf{Client stores:}
\State Client model parameter: $X_n$
\State Client previous model parameter: $X_{n0}$
\Statex
\Procedure {FedDiff}{$\eta$, $T$, $X_0$}
\State \textbf{Initialize:}
\State $\quad \quad X_c, X_n \leftarrow X_0 \quad \forall n = 1, 2, ..., N$
\For {each round $t = 1, 2, ..., T$}
\For {each client $n = 1, 2, ..., N$ \textbf{in parallel}} 
\State \textproc{LocalUpdate}$(B, E, n)$
\State \textproc{ParameterExchange}$(n, X_c)$
\Comment{The order of clients doing \textproc{ParameterExchange} can be different based on different asynchronous scheme}
\EndFor
\EndFor
\EndProcedure
\Statex
\Procedure {LocalUpdate}{$B, E, n$} \Comment{for client $n$}
\State $\mathcal{B} \leftarrow$ split $\mathcal{D}_n$ into batch size of $B$
\State $X_{n0} \leftarrow X_n$
\For{local epoch from 1 to $E$}
\For{batch $b \in \mathcal{B}$}
\State $X_n \leftarrow X_n - \eta \nabla l(X_n; b)$
\EndFor
\EndFor
\State Calculate $\Delta X = X_n - X_{n0}$
\EndProcedure
\Statex
\Procedure {ParameterExchange}{$n, X_c$} \Comment{for client $n$}
\While {}
\State Send current $X_c$ to client $n$
\State Receive $\Delta X$ from client
\State Update $X_c \leftarrow X_c + \frac{\Delta X}{N}$
\EndWhile
\Repeat
\State Send $\Delta X$ to server
\State Receive current $X_c$ from server
\State Update $X_n \leftarrow X_c + \frac{\Delta X}{N}$
\Until {}
\EndProcedure
\end{algorithmic}
\end{algorithm}

% \subsection{The Improved \texttt{FedDiffI} Algorithms}
The most na\"ive schedule for device updates is a cyclic one, in which each device communicates in a pre-set order that does not vary over the communication rounds. If we use the cyclic scheme to update the model parameters, the staleness of the previous model parameters, i.e., the number of global updates that a client misses between its local update transmissions, remains the same for all clients in all communication rounds. However, if we use a \textit{randomized} scheme to schedule the local clients, the staleness will likely be different at each time. Thus, we introduced the improved version of FL algorithms \texttt{FedDiffI}, with the full algorithm shown in Algorithm \ref{alg:FedDiffI}. The key idea is to utilize the staleness as a means of calculating the weight of different local models.

In \texttt{FedDiffI}, the server needs to store the last model parameters $X_{cn}$ of each client $n$, and the timestamp $t_n$ of the model. The weight $u_n(t_n)$ of client $n$'s model parameters $X_{cn}$ is then calculated based on the staleness. The older the model is, the smaller the weight is: intuitively, updates from a more stale model are less likely to be relevant to the current model, and thus should be weighted less~\cite{xie2019asynchronous}. In order to maintain the scale of the model parameters, $u_n(t_n)$ is normalized, i.e., $\sum_{n=1}^N u_n(t_n)=1$. For example, one of the weight we used in the experiment is:

\begin{equation}
    u_n(t_n) = \frac{\frac{1}{(t_c-t_n)^2}}{\sum_{k=1}^N\frac{1}{(t_c-t_k)^2}} 
\end{equation}

Where $t_c$ is the current time.
%\carlee{what $u_n$ did you use in the experiments? give an example here}


\begin{algorithm}
\caption{\texttt{FedDiffI}: There are $N$ clients indexed by $n$, $\eta$ represents the learning rate, $B$ is the batch size, $E$ is the number of local epoch.}
\label{alg:FedDiffI}
\begin{algorithmic}[1]
\State \textbf{Server stores:}
\State Each client's latest model parameter: $X_{cn} \quad \forall n =1, 2, ..., N$
\State Each client's latest model timestamp: $t_n \quad \forall n = 1, 2, ..., N$
\Statex
\State \textbf{Client stores:}
\State Client model parameter: $X_n$
\State Client previous model parameter: $X_{n0}$
\Statex
\Procedure {FedDiffI}{$\eta$, $T$, $X_0$}
\State \textbf{Initialize:}
\State $\quad \quad X_{cn}, X_n \leftarrow X_0 \quad \forall n = 1, 2, ..., N$
\State $\quad \quad t_n \leftarrow 0 \quad \forall n = 1, 2, ..., N$
\For {each round $t = 1, 2, ..., T$}
\For {each client $n = 1, 2, ..., N$ \textbf{in parallel}} 
\State \textproc{LocalUpdate}$(B, E, n)$ \Comment{Same as \texttt{FedDiff}}
\State \textproc{ParameterExchange}$(n, X_c)$
\Comment{The order of clients doing \textproc{ParameterExchange} can be different based on different asynchronous scheme}
\EndFor
\EndFor
\EndProcedure
\Statex
\Procedure {ParameterExchange}{$n, X_c$} \Comment{for client $n$}
\While {}
\State Calculate $X_c = \sum_{n =1}^N u_n(t_n)X_{cn}$ \Comment{$u_n(t_n)$ is the normalized weight calculate from the staleness $t_n$, where $\sum_{n =1}^N u_n(t_n)=1$}
\State Send current $X_c$ to client $n$
\State Receive $\Delta X$ from client
\State Update $X_{cn} \leftarrow X_{c} + \frac{\Delta X}{N}$
\EndWhile
\Repeat
\State Send $\Delta X$ to server
\State Receive current $X_c$ from server
\State Update $X_n \leftarrow X_c + \frac{\Delta X}{N}$
\Until {}
\EndProcedure
\end{algorithmic}
\end{algorithm}





==> 04_quantization.tex <==
% \subsection{Dual-Precision Integer}\label{sec:quantized}
% We observe that the weights and gradients have different precision requirements. 
% One the one hand, large weights are more important then weights that are close to zeros for the model performance as they contribute more to the final outcomes~\cite{han2015deep}. On the other hand, capturing small gradients are crucial in terms of training the model and updating the weights. . 

% \subsection{Server-Assist Adaptive Rescaling}\label{sec:rescale}

% In this section, we outline the key principles underlying the design of quantized neural network training for on-device applications. Leveraging these principles, we illustrate the effective implementation of complete quantized training - including both forward and backward propagation - on devices like the Adafruit Feather M0. These devices are featured with a Cortex M0 microprocessor and are characterized by their modest memory capacity of 32 KB. 

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{figs/quantization.png}
%     \caption{On-device quantized training.}
%     \label{fig:quantization}
% \end{figure}


% \textbf{Stochastic Rounding}
% To effectively train neural networks using low-precision representations of weights, a crucial step involves employing a rounding function to transform real-valued numbers into their quantized counterparts. A common method is deterministic rounding, which rounds a floating point value $v$ to the nearest quantized value. This is represented as $Q_d(v)=\text{sign}(v)\lfloor v+0.5\rfloor$. However, deterministic rounding has limitations, particularly when the magnitude of gradient updates is significantly smaller than the quantization step size, leading to the potential loss of important gradient information.

% To overcome this challenge, we adopt stochastic rounding, which rounds a value to its adjacent quantization levels with a probability  proportionate to its proximity to these levels.  Mathematically, 
% $$Q_s(v) = \begin{cases}\lfloor v \rfloor & p<v - \lfloor v \rfloor ,\\\lfloor v \rfloor + 1 & \text{otherwise},
% \end{cases}$$
% where $p$ is a uniform random number in $[0,1]$. This approach significantly reduces the loss of information in scenarios where small gradient values are involved. 

% % \carlee{need to add citations to this section. It's not clear what is new}

% \begin{figure*}
%     \centering
%     \includegraphics[width=.8\linewidth]{figs/comm.png}
%     \caption{An example round of data transmission in Feather-COMM, with the uplink and downlink model updates each split into four packets. \texttt{up\_status} and \texttt{down\_status} respectively indicate whether each packet has been received yet by the server or device. Status packets are indicated by notched arrows, while data packets are rectangular arrows. Transmission is successful when all four packets are successfully received at the device and at the server.}
%     \label{fig:comm}
% \end{figure*}


% \section{Feather-Comm} \label{sec:comm}
% This section introduces Feather-COMM, a communication protocol designed to optimize federated learning  in IoT  networks. The primary aim of Feather-COMM is to extend the longevity of FL operations and facilitate continual, life-long learning in these networks.


% \subsection{Sparse Model Update} 
% Sending model parameters can be hard for embedded IoT devices, as even a moderate sized model can contain thousands of parameters  and takes a few seconds to send in a low-bandwith network.  In order to further reduce the communication cost from the device side, we consider only transmitting the differences or deltas of the model parameters.  This is based on the observations that most of the gradient updates are close to zero. To implement sparsity in model updates, devices calculate the difference in parameters before and after executing local gradient descent. Only those parameters with changes greater than zero are transmitted. This approach necessitates maintaining a buffer on the device to store the last received model from the server. Through this differential calculation, devices can efficiently package and transmit only those parameters that exhibit significant changes.

% \textbf{Binary Coding} We've developed a compact binary coding scheme for sending these updates. In this scheme, only the parameters with non-zero changes are transmitted, along with a bitmap that indicates which parameters are included. This approach ensures that the server knows exactly which parameters have been updated. For successful decoding and application of these updates, it's essential that both the devices and the server agree on a specific order for processing the model parameters.
 
%  In this scheme, gradients with zero change incur a minimal communication cost of just 1 bit. In contrast, non-zero quantized gradients require a slightly higher cost of $b+1$ bits where $b$ is the number of bits representing the gradient parameter. Consequently, the sparser the update (i.e., the fewer non-zero changes), the fewer bits are needed for transmission. This approach draws inspiration from frequency-based encoding methods, where more common data (in this case, zero gradients) are encoded using fewer bits, thereby achieving greater communication efficiency.
 
% \textbf{Thresholding} In addition to avoid sending zero difference, we can further sparsify the model difference by only sending updates that are greater than some threshold. In this way, we are introducing more errors by ignoring small parameter updates from the devices, while further reducing the communication cost. By adjusting this threshold value, we are able to tradeoff between communication and learning performance (Section \ref{sec:tradeoff}).
